FLEX: Extrinsic Parameters-free Multi-view 3D Human Motion Reconstruction

The increasing availability of video recordings made by multiple cameras has offered new means for mitigating occlusion and depth ambiguities in pose and motion reconstruction methods. Yet, multi-view algorithms strongly depend on camera parameters; particularly, the relative transformations between the cameras. Such a dependency becomes a hurdle once shifting to dynamic capture in uncontrolled settings. We introduce FLEX (Free muLti-view rEconstruXion), an end-to-end extrinsic parameter-free multi-view model. FLEX is extrinsic parameter-free (dubbed ep-free) in the sense that it does not require extrinsic camera parameters. Our key idea is that the 3D angles between skeletal parts, as well as bone lengths, are invariant to the camera position. Hence, learning 3D rotations and bone lengths rather than locations allows predicting common values for all camera views. Our network takes multiple video streams, learns fused deep features through a novel multi-view fusion layer, and reconstructs a single consistent skeleton with temporally coherent joint rotations. We demonstrate quantitative and qualitative results on three public datasets, and on synthetic multi-person video streams captured by dynamic cameras. We compare our model to state-of-the-art methods that are not ep-free and show that in the absence of camera parameters, we outperform them by a large margin while obtaining comparable results when camera parameters are available. Code, trained models, and other materials are available on our project page.

==> figures/ablation_fusion_layer_reduced.tex <==
% \begin{wraptable}{r}{4.5cm}
\begin{center}
\begin{tabular}{|c|c|} \hline

%\makecell{\textbf{2D from} $\rightarrow$ \\ \textbf{\#Views}\downarrow$}& \textbf{GT } & \textbf{\cite{iskakov2019learnable}}\\
\textbf{Method} & \textbf{MPJPE } \\
\hline
\makecell{Avg. \\ $K$ views} & 36.4 \\
\hline
\makecell{Late \\ fusion} & 31.0 \\
\hline
FLEX & \textbf{24.8} \\
\hline
\end{tabular}
\end{center}
% \caption{The impact of various fusion methods. Note that processing all views together with an early fusion as performed in FLEX outperforms the other variations by a large margin.}
\label{tab:ablation}
% \end{wraptable}


==> figures/generalization.tex <==
\begin{figure}[tbh]
\centering
\setlength{\abovecaptionskip}{0pt plus 3pt minus 2pt}
\setlength{\belowcaptionskip}{-10pt plus 3pt minus 2pt}
\caption*{}

% \includegraphics[width=.9\linewidth]{./images/rebutall_2cams.jpg}
\includegraphics[width=.9\linewidth]{./images/rebutall_2cams_b.png}

\setlength{\abovecaptionskip}{-10pt plus 3pt minus 2pt}
\setlength{\belowcaptionskip}{-20pt plus 3pt minus 2pt}

\caption{
%Generalization: 
Evaluation on two cameras, while training on two others.}
% (a) evaluation on the Ski-pose dataset. (b) evaluation on 2 cameras, while training on 2 others.}
\label{fig:general}

\end{figure}

==> figures/global_mpjpe_table.tex <==

\begin{table}[tb]
\color{red}
\begin{center}
\caption{Global MPJPE error on Human3.6M.
Legend:$(*)$ is a non ep-free algorithm.}
\begin{tabular}{|c|c|}
\hline
\textbf{Method} & \textbf{MPJPE} \\ \hline
\makecell{Iskakov\cite{iskakov2019learnable}$(*)$ \\ param. perturb by 3\%} & 123 \\ \hline
FLEX & \textbf{118} \\ \hline

\end{tabular}
\label{tab:global_mpjpe}
\end{center}


\end{table}


==> figures_unused/ablation_mha_heads.tex <==
% \begin{table}[tb]
% \color{orange}
% % \begin{wraptable}{r}{4.5cm}
% % \vspace{-25pt}
% \begin{center}
% \begin{tabular}{|c|c|}
% \hline
% \textbf{Method} & \textbf{MPJPE} \\

% \hline
% Convolution layer & 31.9 \\
% \hline
% Transformer Encoder - 1 layer, 64 heads & 30.95 \\
% \hline
% Transformer Encoder - 2 layers, 64 heads & 37.81 \\
% \hline
% Multi-head Attention - 128 heads & 30.5 \\
% \hline
% Multi-head Attention - 64 heads & \textbf{30.18} \\
% \hline
% Multi-head Attention - 32 heads & 30.62 \\
% %\hline
% %Multi-head Attention - 16 heads & 30.86 \\
% \hline

% \end{tabular}
% \end{center}
% \vspace{-14pt}
% % \caption{The impact of different configurations on our multi-view fusion layer. }
% \caption{The impact of multi-view fusion architecture. }
% \label{tab:ablation_mha_heads}
% % \end{wraptable}
% \vspace{-5pt}
% \end{table}

\begin{table}[t]
\color{orange}
% \begin{wraptable}{r}{4.5cm}
% \vspace{-25pt}
\begin{center}
\begin{tabular}{|c|c|}
\hline
\textbf{Method} & \textbf{MPJPE} \\

\hline
Conv. layer & 31.9 \\
\hline
TE - 1$l$, 64$h$ & 30.95 \\
\hline
TE - 2$l$, 64$h$ & 37.81 \\
\hline
MHA - 128$h$ & 30.5 \\
\hline
MHA - 64$h$ & \textbf{30.2} \\
\hline
MHA - 32$h$ & 30.6 \\
\hline
MHA - 16$h$ & 30.9 \\
\hline

\end{tabular}
\end{center}
\vspace{-14pt}
\caption{The impact of multi-view fusion architecture. Legend: TE - Transformer Encoder. MHA - Multi-head Attention. $l$ refer to no. of stacked layers. $h$ refer to no. of heads in attention layer.}
\vspace{-5pt}
\label{tab:fusion_arch}
% \end{wraptable}
\end{table}

==> figures_unused/competitors.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{./images/competitors_grid.jpg}
\vspace{-20pt }
\caption{
%\color{orange}Frames from the H3.6M dataset. Shows the strenghts of our work. Predicting bones and rotations help to receive a more smooth motion. At Iskakvot \etal~\cite{iskakov2019learnable} column we can see the at the first row we received a huge right leg, and at the third colum the left elbow is rotated inside in a non-natural way. Comparing our results against Shi \etal~\cite{shi2020motionet} we show the benefits of our multi-view algorithm that produces more accurate results.}
Qualitative comparison of our work vs. non ep-free state-of-the-art (Iskakov \etal~\cite{iskakov2019learnable}) and vs. our single-view baseline (Shi \etal~\cite{shi2020motionet}).}
\label{fig:competitors}
\ifeccv
\else
\vspace{-17pt}
\fi
\end{figure}

==> figures_unused/fight_results.tex <==
\begin{figure*}[htb]
\centering
\includegraphics[width=\linewidth]{./images/Fight_results.pdf}
\caption{\brr{Fight results }}
\label{fig:fight_results}

\end{figure*}


==> figures_unused/football_teaser.tex <==
% \begin{teaserfigure}
\begin{figure}
\centering
\includegraphics[width=\linewidth]{./images/football_results.pdf}
\vspace{-17pt}
\caption{Motion reconstruction on the KTH Multi-view Football II dataset~\cite{footballDS} in occluded and blurry scenes. 
Each row depicts three views of one time frame. 
To the right of each image we put a reconstructed rig of the player. % \#20. 
The KTH dataset is filmed using moving cameras, hence camera extrinsic parameters vary between frames. 
FLEX is ep-free, so it is agnostic to camera parameters and is not affected by the change in their values.
}
%does not require the acquaintance of camera parameters.

% Our algorithm is agnostic to the lack of camera parameters since it does not apply triangulation nor projection.} 
%\dc{How about: Our algorithm is ep-free, since it is agnostic to the lack of camera parameters. Or, since it does not rely on the camera parameters.}}
\label{fig:football_teaser}
% \end{teaserfigure}
\vspace{-10pt}

\end{figure}



==> figures_unused/macarena_results.tex <==
\begin{figure*}[htb]
\centering
\includegraphics[width=\linewidth]{./images/Macarena_results.pdf}
\caption{\brr{Macarena results }}
\label{fig:macarena_results}
\iftog{}\else{
\vspace{-5pt }% save space (but for tog it looks bad)
}\fi
\end{figure*}

==> figures_unused/qualitative.tex <==
\iftog
\begin{figure*}[tbh]
\else
\begin{figure}[t]
\fi
\centering
\includegraphics[width=\linewidth]{./images/H36M_results.pdf}
\vspace{-20pt}
\caption{Our results on videos from the Human3.6M dataset. }
\label{fig:quality_h36}
\iftog
\end{figure*}
\else
\vspace{-5pt}
\end{figure}
\fi

% \ifcvpr 
\ifeccv{}\else{
\begin{figure}[tb]
\vspace{-10pt}
\centering
\includegraphics[width=\linewidth]{./images/football_results.pdf}
\vspace{-15pt}
\caption{Our results on videos from the more challenging KTH Multi-view Football II dataset. Notice how we mitigate occlusion and blurriness in the middle row.}
\label{fig:quality_KTH}
\vspace{-10pt}
\end{figure}
}
\fi
% \input{./figures/blender_studio}
% \input{./figures/fight_results_with_circles}
% \input{./figures/macarena_results_with_circles}



==> figures_unused/quantitative_acc_error.tex <==
\begin{table}[tb]
\begin{center}
\begin{tabular}{|c|c|}
\hline
\textbf{Method} & \textbf{Acc. Error} \\ \hline
VIBE\cite{kocabas2020vibe} & 18.3 \\ \hline
MEVA\cite{luo20203d} & 15.3 \\ \hline
HMMR\cite{kanazawa2019learning} & 9.1 \\ \hline
TCMR\cite{choi2021static} & 5.3 \\ \hline
Iskakov \etal~\cite{iskakov2019learnable} & 3.9\\ \hline
FLEX ($\star$) & \textbf{1.6} \\ \hline
FLEX ($\bullet$) & \textbf{0.9} \\ \hline

\end{tabular}
\end{center}
\vspace{-15pt}
\caption{Smoothness, measured by acceleration error in $mm/s^2$,  on Human3.6M (lower is better). Legend: ($\star$) Using \cite{iskakov2019learnable} for 2D pose backbone. ($\bullet$) Using ground-truth 2D poses.}
\label{tab:acc_error}
\vspace{-10pt}
\end{table}

% \begin{table}[tb]
% \color{orange}
% \begin{center}
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \textbf{Method}  & \cite{luo20203d} & \cite{kanazawa2019learning} & \cite{choi2021static} & \cite{iskakov2019learnable} &($\star$) & ($\bullet$) \\ \hline

% \textbf{Acc. Error} 
% %  & 18.3 
%  & 15.3  
%  & 9.1  
%  & 5.3  
%  & 3.9 
%  & \textbf{1.6}
%  & \textbf{0.9} \\ \hline

% \end{tabular}
% \end{center}
% \vspace{-15pt}
% \caption{\color{orange} Smoothness, measured by acceleration error in $mm/s^2$,  on Human3.6M (lower is better). Legend: ($\star$) FLEX using \cite{iskakov2019learnable} for 2D pose backbone. ($\bullet$) FLEX using ground-truth 2D poses.}
% \label{tab:acc_error}
% \vspace{-10pt}
% \end{table}



==> figures_unused/quantitive_solvePNP_error.tex <==
\begin{table}
\begin{center}

\begin{tabular}{c}
$R$\\
\end{tabular}
\begin{tabular}{|ccc|}
\hline
  0.3 & -1.3 & -2.3 \\
% \hline
-22.5  & -8.9 &  0.5 \\
% \hline
 -1.1 &  0.8 & -9.4 \\
\hline
\end{tabular}
% \quad
\\
\vspace{1mm}
\begin{tabular}{c}
$T$\\
\end{tabular}
\begin{tabular}{|ccc|}
\hline
-110.1 & -100.6 & 316.5\\
\hline
\end{tabular}
\\

\vspace{1mm}
\begin{tabular}{c}
$K$\\
\end{tabular}
\begin{tabular}{|cccc|}
\hline
-110.1 & -100.6 & 316.5\\
\hline
-110.1 & -100.6 & 316.5\\
\hline
\end{tabular}
\end{center}
% \caption{Mean error percentage when estimating $R$ and $T$ using opencv::solvePnP.}
\label{tab:cv2_pnp_err}
\iftog{}\else{
\vspace{-5pt }% save space (but for tog it looks bad)
}\fi
\end{table}



==> figures_unused/rebuttal_epipolar_transformers.tex <==
\begin{figure}[b]
\vspace{-5pt}
\centering
\includegraphics[width=\linewidth]{./images/rebuttal_epipolar_transformers1.jpg}
\vspace{-20pt}
\caption{
In a cross-view attention, attended keys should be taken evenly from all views. 
Epipolar Transformers (left): spatial-attention across locations on an epipolar line in a single view.
Ours (right): view-attention across all views.
%Left: attend spatial points in the epipolar line in view 2 to best match the 2D joint in view 1. Right: attend views to best match 3D ground-truth joint rotation.
} 
\label{fig:rebuttal_epipolar_transformers}
\vspace{-5pt}
\end{figure}


==> figures_unused/rebuttal_root_pos.tex <==
\begin{figure}[b]
\centering
% \includegraphics[width=\linewidth]{./images/rebuttal_3d_root_position.png}
\includegraphics[width=\linewidth]{./images/root_positions_color.jpg}
\vspace{-20pt}
\caption{ 
Positions of the root coordinate along time: 
GT is depicted in thin black.  
Our scaled prediction is in an overlay on top of the GT, with  'S' and 'E' stating where the start and the end are, respectively.
%, and changes from yellow to red when time progresses. 
Depicted motions are (Human3.6M -- left to right): walk, phone, eat.
}
\label{fig:root_pos}
\vspace{-5pt}
\end{figure}

% The angle of view is selected to obtain the best visualization, and scaling is applied to overcome weak perspective. 


==> figures_unused/rebuttal_ski_ptz_qualitative.tex <==
\begin{figure}[tb]
\centering
\includegraphics[width=\linewidth]{./images/Ski_results_3_rows_B.jpg}
\vspace{-20pt}
\caption{Our results on videos from the Ski-Pose PTZ-Camera dataset.} 
\label{fig:ski_ptz_qualitative}
\vspace{-10pt}
\end{figure}



==> figures_unused/tables_ablation_fusion_mha_heads.tex <==
\begin{table}[!htb]
    \begin{minipage}{.45\linewidth}
      \centering
        \ifeccv
        \caption{The impact of multi-view fusion architecture. Legend: TE - Transformer Encoder. MHA - Multi-head Attention. $l$ refer to no. of stacked layers. $h$ refer to no. of heads in attention layer.}
        \fi
        \input{./figures/ablation_mha_heads_reduced}
        \ifeccv
        \else
        % \vspace{-5.8pt}
        \caption{The impact of multi-view fusion architecture. Legend: TE - Transformer Encoder. MHA - Multi-head Attention. $l$ refer to no. of stacked layers. $h$ refer to no. of heads in attention layer.}
        \fi
        \label{tab:num_views}
    \end{minipage}%
    \hspace{.1\linewidth}
    \begin{minipage}{.45\linewidth}
      \centering
      \ifeccv
      \caption{The impact of various fusion methods. Note that processing all views together with an early fusion as performed in FLEX outperforms the other variations by a large margin.}
      \fi
      \input{./figures/ablation_fusion_layer_reduced}
      \ifeccv
      \else
      \vspace{-12pt}
      \caption{The impact of various fusion methods. Note that processing all views together with an early fusion as performed in FLEX outperforms the other variations by a large margin.}
      \fi
      \label{tab:2D_backbone}
    \end{minipage} 
\vspace{-13pt }
\end{table}

==> sup_mat/sup_network_structure.tex <==
\input{LaTeX/figures/layer_detail}


\sout{We now describe the full architecture of each component, $F_Q$, $E_Q$, $F_S$, $E_S$ and $D$. The parameters of each layer are detailed in \cref{tab:layer_detail}.

Both fusion components $F_Q$ and $F_S$ start with a channel-expansion layer, followed by a view-fusion block, and completed by a transformer encoder {\color{orange}multi-head attention layer} that attends views.}
%In both $F_S$ and $F_Q$ there are three main parts: channel-expansion, information-fusion and view-wise attention.
\sout{
Channel-expansion is done using convolutional layers with a kernel of size 1.
%In the expansion part we use convolutional blocks, where the convolutions have kernel size 1 and stride 1. 
In the view-fusion part, for $F_Q$, we apply three parallel 2D convolutional kernels with different kernel sizes, followed by adaptive average pooling. For $F_S$, we use sequential convolutional layers.

Our view-transformer block is based on the  LiftFormer transformer encoder and contains two transformer encoder layers with two heads each. Each transformer encoder is composed of two self attention layers with layer norm. 
The result of applying the view-transformer is that the view dimension collapses (visualized in \cref{fig:architecture_detail}).}
{\color{orange}\sout{
Our view-attention block is composed of 64 attention heads. The result of applying the view-attention is that the view dimension collapses (visualized in \cref{fig:architecture_detail}).}}

\sout{The encoder block $E_Q$ consists of three parallel 1D convolutional layers of different kernel sizes, followed by a final additional 1D convolution. The encoder $E_S$ starts with an adaptive max pooling to collapse the time dimension and then runs a final 1D convolution.

%and then collapse all the temporal information into a single vector with adaptive max pooling. Then for both branches we apply a view-wise transformer encoder composed of 2 layers that each contains a 2-heads attention block.
 
Our discriminator $D$ is a linear component that contains two convolution layers and one fully connected layer, based on Kanazawa~\etal~\shortcite{Kanazawa:2018}). Its output value is between 0 and 1.  
%for each rotating joint, that is, a joint that is not an end effector.as there are joints that are end-effectors which means they don't have any rotation in the human kinematic chain, so their rotation angle is not predicted by our network. 
 
After each convolution block, we apply batch normalization, a leaky rectified linear unit and dropout. 
%The kernel width and the stride are denoted by $k$ and $s$, respectively, and the number of input and output channels is given in the rightmost column.}{}
}


